Disentangling Reasoning Tokens and Boilerplate Tokens For Language Model Fine-tuning

When using agent-task datasets to enhance agent capabilities for Large Language Models (LLMs), current methodologies often treat all tokens within a sample equally. However, we argue that tokens serving different roles - specifically, reasoning tokens versus boilerplate tokens (e.g., those governing output format) - differ significantly in importance and learning complexity, necessitating their disentanglement and distinct treatment. To address this, we propose a novel Shuffle-Aware Discriminator (SHAD) for adaptive token discrimination. SHAD classifies tokens by exploiting predictability differences observed after shuffling input-output combinations across samples: boilerplate tokens, due to their repetitive nature among samples, maintain predictability, whereas reasoning tokens do not. Using SHAD, we propose the Reasoning-highlighted Fine-Tuning (RFT) method, which adaptively emphasizes reasoning tokens during fine-tuning, yielding notable performance gains over common Supervised Fine-Tuning (SFT).

==> section/preliminaries.tex <==
\section{Preliminary Considerations: Characteristics of Tool-Use Data}
In this section, we present our analysis of two pivotal attributes of the Tool-use Data for agents and illustrate how they undermine the accuracy of data selection tailored for general instruction calibration.


\textbf{Strict format .} The majority of research on tool-use employs a stringent, uniform format for prompting the agent. This approach is deemed appropriate for the purposes of inference; however, it may be less than optimal when considering the nuances of training and data selection.

The datasets employed in recent studies~\cite{qin_toolllm_2023,zeng_agenttuning_2023,yao_react_2023} are tailored to conform to specific structural formats, most notably with JSON format in response. This standardization facilitates efficient parsing and interpretation of the data and additionally directs the computational models' approach towards solving the problems effectively. Nonetheless, the uniformity and inherent simplicity associated with format learning could inadvertently engender a bias within the method of data selection. This inclination may lead to the preferential choice of datapoints that share similar format with the target data.
% TODO: hard data sel?
\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{figure/format_overlap.pdf}
    \caption{overlap rate of data selected by LESS use different format on same target data question}
    \label{fig:format-overlap}
\end{figure}

\textbf{Multi-step .} Owing to the inherent complexity exhibited by most agent tasks, they necessitate a multi-step process involving critical thinking, tool utilization, and feedback-based learning. The impact of preceding steps must be considered a crucial metric for evaluating the quality of an agent's data.



Unlike the instruction-tuning data typically employed in prior research, which generally involves only a single-turn dialogue~\cite{DatabricksBlog2023DollyV2,taori2023alpaca,longpre_flan_2023}, multi-step interactions are a critical feature of agent data, essential for enhancing LLMs capabilities in planning, stepwise reasoning, summarization, and feedback learning~\cite{lightman_lets_2023,zeng_agenttuning_2023}. Merely adopting previous methods for multi-step data results in an overemphasis on the initial step, while neglecting subsequent steps and the connections between them.

\input{table/truncate_overlap}
